Strategy-Stealing is Non-Constructive

In many combinatorial games, one can prove that the first player wins under best play using a simple but non-constructive argument called strategy-stealing. This work is about the complexity behind these proofs: how hard is it to actually find a winning move in a game, when you know by strategy-stealing that one exists? We prove that this problem is PSPACE-hard already for Minimum Poset Games and Symmetric Maker-Maker Games, which are simple classes of games that capture two of the main types of strategy-stealing arguments in the current literature.

==> oldtext.tex <==
%%%THIS FILE CONTAINS THINGS I DIDN'T WANT TO DELETE, BUT THAT I DON'T THINK ARE RELEVANT ANYMORE


\iffalse
\begin{proof}
Given an instance $Q$ of $\textsc{DecisionHex}$, we define a symmetric maker-maker game as follows.
We will call the players \emph{red} and \emph{blue}, and suppose it is currently red's turn to move.
We make three copies of the game board $Q_1, Q_2, Q_3$, and we also add six auxiliary elements to the game, $r_1, r_2, r_3, b_1, b_2, b_3$. We refer to $r_1, r_2$ and $r_3$ as the \textit{red elements}, and $b_1, b_2, b_3$ as the \textit{blue elements}. We refer to all six of these elements collectively as the \textit{gadget elements}.
The winning sets in the new game are:
\begin{itemize}
    \item Any set of hexes that would complete a win for the red player on $2$ of the $3$ boards (if all colored red), as well as two of the three elements $r_1, r_2, r_3$ or
    \item Any set of elements that would complete a win for the blue player on $2$ of the $3$ boards (if all colored blue), together with (at least one) set of the form $\{b_i, b_j, r_i\},$ with $i \neq j$, or the set $\{b_1, b_2, b_3\}$.
    %\item
    %For any $i$ and $j$ (with $i \neq j$), the set $\{r_i, b_i, r_j\}$.
    \item
    Any subset of size at least 4 of $\{r_1, r_2, r_3, b_1, b_2, b_3\}$ which contains at least two of $\{r_1, r_2, r_3\}$.
\end{itemize}
We will call these types \emph{red} winning sets, \emph{blue} winning sets, and neutral winning sets (respectively).
The players in this new game are $p_1, p_2$ with $p_1$ moving first.
Our goal is to argue that it is a winning strategy for $p_1$ to take a blue element with their first move if and only if $Q$ is a win for blue.
We break this down into cases as follows.
\begin{lemma}
Blue has a winning strategy in $Q$, if and only if the only winning first moves for $p_1$ are claiming either $b_1, b_2,$ or $b_3$
\end{lemma}
\begin{proof}
We first show that if Blue has a winning strategy in $Q$, then by claiming one 
of $b_1, b_2,$ or $b_3$, player $p_1$ can win. Suppose without loss of generality that $p_1$ played $b_1$. The strategy for $p_1$ after the first move will be as follows: 

\begin{itemize}
\item 
Throughout the whole game, every time the opposing player $p_2$ plays on one of $Q_1, Q_2$ or $Q_3$, player $p_1$ will play on the same board $p_2$ just played on, according the Blue's winning strategy on that board. 
\item
If the opposing player claims a blue element ($b_2$ or $b_3$), then claim the remaining blue element (suppose $b_2$, without loss of generality). Then, the next time the opposing player claims an element from the gadget, claim either $r_1$ or $r_2$ (whichever is available).
\item
If the opposing player $p_2$ plays $r_1$, claim $b_2$. Then, the next time the opposing player claims either an $r_i$ or $b_i$, claim either $r_2$ or $b_3$, whichever is available. 
\item
If the opposing player plays $r_2$ or $r_3$, claim $b_2$, Then, the next time $p_2$ claims some $b_i$ or $r_i$, claim the remaining one of $r_1$ or $b_3$.
\end{itemize}


%they can then only try for blue winning sets, and make each move on the same board on which $p_2$ made their last move.

We will now prove that the above is indeed a winning strategy. First, note that by the assumption that Blue has a winning strategy in $Q$, and the fact that whenever $p_2$ plays on one of the boards $Q_i$, player $p_1$ responds with Blue's winning move on that board, we know that it is impossible for $p_2$ to obtain a red winning set. Additionally, notice that it is impossible for $p_2$ to obtain a blue winning set, since $p_1$ begins by claiming a blue element, then if $p_2$ claims a blue element, $p_1$ responds by taking  the remaining blue element (and at least two blue elements are needed to obtain a blue winning set, so $p_2$ cannot obtain a blue winning set). Notice also that $p_2$ cannot obtain a neutral winning set, since $p_1$ always secures at least three of the gadget elements. %, and then wins in the next move (notice that $p_2$ will need $3$ elements from the gadget in order to obtain a blue winning set, but $p_1$ will win after the next move so $p_2$ will not have enough moves available to claim a blue winning set). It is also impossible for $p_2$ to obtain a neutral winning set, since if $p_2$ claims a blue element, as we've seen $p_1$ will obtain a neutral winning set (note that at most one player can obtain a neutral winning set, since a neutral winning set requires two red elements), and if $p_2$ claims a red element then within two moves $p_1$ will have either all three blue elements, or a triple of the form ${b_i, b_j, r_k}$ (where $i, j, k$ are all different). Once $p_1$ has that, it is impossible for $p_2$ to obtain a neutral winning set.


We now will show that $p_1$ will obtain a winning set. Notice that on the boards $Q_1, Q_2, Q_3$, the first player $p_1$ will obtain a win for Blue (since by assumption Blue as a winning strategy, and on the boards $Q_1, Q_2, Q_3$ the player $p_1$ responds to all moves of $p_2$ with the corresponding move which is optimal for $p_1$. So, we are left to show that $p_1$ will obtain a triple of the form $\{b_i, r_i, b_j\}$, since that is what is left to secure a blue winning set. We will focus on moves that claim a gadget element (one of the $r_k$ or $b_k$), since for other moves on the boards $Q_i$, the player $p_1$ responds with a move on the board. If $p_2$ claims a blue element, then $p_1$ responds by claiming the remaining blue element $b_{\ell}$. Then, the next time $p_2$ claims a gadget element, $p_1$ will take either $r_1$ or $r_{\ell}$, whichever is available, now securing a triple $\{b_i, r_i, b_j\}$. If $p_2$ claims the red element $r_1$, then $p_1$ will claim $b_2$, and then the next time $p_2$ claims a gadget element, $p_1$ claims either $b_3$ or $r_2$, whichever is left (thus securing a triple  $\{b_i, r_i, b_j\}$ or $\{b_1, b_2, b_3\}$). If the $p_2$ claims $r_2$ or $r_3$, then $p_1$ claims $b_2$, and then the next time $p_2$ claims a gadget element, $p_1$ claims either $r_1$ or $b_3$, whichever is left (thus securing a triple  $\{b_i, r_i, b_j\}$ or $\{b_1, b_2, b_3\}$).

If $p_2$ claims a red element, then we have seen that within two moves $p_2$ will obtain a triple ${b_i, b_j, r_k}$ (where $i, j, k$ are all different). Additionally, $p_1$ will eventually obtain a winning combination for blue on all 3 of the boards, since, whenever $p_2$ plays on one of the boards, $p_1$ will play on it according to Blue's winning strategy, then $p_1$ will obtain a blue winning set. Every time $p_1$ claims a gadget element, $p_2$ responds by claiming a gadget element, so also $p_1$ cannot obtain a neutral winning set.


We will now show that other than claiming a blue element, there is no other winning move for $p_1$. Suppose that $p_1$ claims a red element $r_i$. Then, $p_2$ can claim $b_i$. Then, in the next move $p_2$ can claim a blue element (there will be at least one blue element remaining). Also, whenever the first player $p_1$ plays on one of the boards $Q_i$, the second player $p_2$ can respond with a winning move for Blue on that board. Because Blue has a winning strategy on the boards, we see that $p_1$ cannot obtain a red winning set. Additionally, the second player $p_2$ will have two blue gadget elements, so the first player $p_1$ will be unable to obtain a blue winning set.

Suppose that the first player claims (as his first move) an element on one of the boards $Q_1, Q_2,$ or $Q_3$ (suppose without loss of generality that the move was on $Q_1$. Then, $p_2$ can respond by claiming $b_1$. Now, whenever $p_1$ plays on either $Q_2$ or $Q_3$, we have $p_2$ respond with a winning move for Blue. By the assumption that Blue has a winning strategy, we see that $p_2$ will have a winning set for Blue in both $Q_2$ and $Q_3$. Therefore, $p_1$ will not have a red winning set, since he will be unable to win as red on at least two of the boards. When $p_1$ claims a gadget element, $p_2$ will respond by claiming a remaining either $b_2$ or $b_3$ (note that at least one of those will remain). Notice now that $p_2$ will have claimed two blue elements, and so $p_1$ will also be unable to obtain a Blue winning set.
%
%
%
%By playing a winning strategy for blue on each board individually, $p_2$ will obtain blue winning sets on all three boards, thus winning the new game.
%
%If $p_1$ does not claim the blue element (but there is a winning strategy for blue), then $p_2$ can win with the following strategy: claim the blue element, and then ignore the board on which $p_1$ made their first move.
%By playing a winning strategy for blue on the remaining two boards, $p_2$ will obtain blue winning sets on both of these boards, thus winning the new game.
\end{proof}

\begin{lemma}
If red has a winning strategy in $Q$, then $p_1$ has at least one winning move, but claiming the blue element with the first move is not a winning move.
\end{lemma}
\begin{proof}


The winning strategy for $p_1$ is as follows. First, claim $r_1$. Now, if $p_2$ does not claim a gadget element, $p_1$ can secure a win by obtaining a neutral set within 3 moves (by repeatedly picking more gadget elements until 4 have been collected, starting with the red elements). So, $p_2$ must respond by picking a gadget element. Then, $p_1$ responds by picking a remaining red gadget element (there must be at least one remaining). $p_2$ must respond by choosing a gadget element (otherwise $p_1$ will be able to obtain a neutral winning set within the next two moves). Then, $p_1$ can claim one of the remaining gadget elements, forcing $p_2$ to claim the last gadget element (to avoid $p_1$ winning via a neutral winning set).

Next, $p_1$ will by play a winning strategy for red on $Q_1$.
If $p_2$ plays on $Q_1$, then continue this strategy.
As soon as $p_2$ plays on a different board -- say, $Q_2$ -- then start playing a winning strategy for red on $Q_3$.
Thus $p_1$ will obtain red winning sets on two of the three boards.

So we have shown that $p_1$ has a winning strategy. We are left to show that $p_1$ does not have a winning strategy that starts with claiming a blue element.


Suppose $p_1$ claims a blue element with their first move. Without loss of generality suppose that $p_1$ claimed $b_1$. Then $p_2$ responds by claiming $r_1$.

There are now two cases. Either $p_1$ chooses a gadget element, or not. First, we examine the case where $p_1$ chooses a gadget element. In this case, $p_1$ either claims a blue element or a red element:

\paragraph{$p_1$ picks a blue element} Suppose $p_1$ responds by claiming another blue element (suppose it is $b_2$ without loss of generality). Then $p_2$ responds by claiming $r_2$. At this point $p_1$ will be unable to secure a red or neutral winning set (because $p_2$ has claimed two red elements). Additionally, if $p_1$ does not claim $b_3$ then he will be unable to secure a blue winning set. So, the only possibly winning move for $p_1$ must be $b_3$. Next, $p_2$ will by play a winning strategy for red on $Q_1$.
If $p_1$ plays on $Q_1$, then continue this strategy.
As soon as $p_1$ plays on a different board -- say, $Q_2$ -- then $p_2$ starts playing a winning strategy for red on $Q_3$.
Thus $p_2$ will obtain red winning sets on two of the three boards (and so $p_1$ will not win, since he will be unable to win as blue on at least two of the boards).

\paragraph{$p_1$ picks a red element} Suppose $p_1$ responds by claiming a red element (suppose it is $r_2$ without loss of generality). Then $p_2$ responds by claiming the remaining red element. At this point $p_1$ will be unable to secure a red or neutral winning set (because $p_2$ has claimed two red elements). Additionally, if $p_1$ does not claim $b_2$ then he will be unable to secure a blue winning set (since in the next move $p_2$ can claim $b_2$). So, the only possibly winning move for $p_1$ must be $b_3$. Next, $p_2$ will by play a winning strategy for red on $Q_1$.
If $p_1$ plays on $Q_1$, then continue this strategy.
As soon as $p_1$ plays on a different board -- say, $Q_2$ -- then $p_2$ starts playing a winning strategy for red on $Q_3$.
Thus $p_2$ will obtain red winning sets on two of the three boards (and so $p_1$ will not win, since he will be unable to win as blue on at least two of the boards).


We are now left with the case that $p_1$, as his second move, picks a non-gadget element. In this case, $p_2$ will respond by claiming $b_2$. Now, $p_1$ must claim a gadget element (otherwise, $p_2$ will be able to claim a neutral winning set within the next two moves by simply claiming whatever gadget elements are left, starting with the red elements). 

\end{proof}

Together, these imply that we can determine the winning player in $Q$ by finding an optimal first move in the new symmetric maker-maker game (in particular, checking whether or not it is to take the blue element).
This completes the reduction.
\end{proof}

\section{New Gadget}

\begin{theorem}
$\P^{\smm} = \PSPACE$.
\end{theorem}
\fi

%It suffices to show that $\textsc{DecisionHex} \in \P^{\smm}$, since $\textsc{DecisionHex}$ is $\PSPACE$-complete CITE.

%Consider an instance $B$ of $\textsc{DecisionHex}$. We will construct a new game (which will be a symmetric maker-maker game, and in the class \smm) based on $B$. The idea for this new game will be that the first player (in his first move) will get to decide if he wants to play as the red player or as the

%The set $X$ of valid moves will consist of the valid moves in $B$, and an additional $6$ elements $r_1, r_2, r_3, b_1, b_2, b_3$. We refer to these $6$ elements as the ``turn gadget''.

%The idea will be that in the first few moves, both players are incentivized to pick elements of the turn gadget. Additionally, we will construct the gadget so that the first player 



\begin{proof}
Given an instance $Q$ of $\textsc{DecisionHex}$, we define a symmetric maker-maker game as follows.
We will call the players \emph{red} and \emph{blue}, and suppose it is currently red's turn to move.
We make a three copies $Q_1, Q_2, Q_3$ of the game board, and we also add five auxiliary elements to the game, $r_1, r_2, b_1, b_2, b_3$. We refer to $r_1, r_2$ and as the \textit{red elements}, and $b_1, b_2, b_3$ as the \textit{blue elements}. We refer to all five of these elements collectively as the \textit{gadget elements}.
The winning sets in the new game are:
\begin{itemize}
    \item Any set of hexes that would complete a win for the red player on 2 of the 3 boards, as well as $r_1$ and $r_2$
    \item Any set of hexes that would complete a win for the blue player on on 2 of the 3 boards, as well as $b_1, b_2$, and $b_3$.
    \item
    $\{r_1,b_1\}, \{r_2, b_2\}$
\end{itemize}
We will call these types \emph{red} winning sets, \emph{blue} winning sets, and neutral winning sets (respectively).
The players in this new game are $p_1, p_2$ with $p_1$ moving first.
Our goal is to argue that it is a winning strategy for $p_1$ to take a blue element with their first move if and only if $Q$ is a win for blue.
We break this down into cases as follows.
\begin{lemma}
Blue has a winning strategy in $Q$, if and only if the only winning first moves for $p_1$ are claiming either $b_1$ or $b_2$.
\end{lemma}
\begin{proof}
We first show that if Blue has a winning strategy in $Q$, then by claiming one 
of $b_1$ or $b_2,$ player $p_1$ can win. Suppose without loss of generality that $p_1$ played $b_1$. Then $p_2$ is forced to play $r_1$ (otherwise, $p_1$ will claim $r_1$ and win with the winning set $\{b_1, r_1\}$. Next, $p_1$ will play $b_2$, and similarly $p_2$ will be forced to play $r_2$. Next, $p_1$ will claim $b_3$. Now, on the boards $Q_1, Q_2$, and $Q_3$, player $p_1$ will respond to each of $p_2$'s moves on a board according to Blue's winning strategy on that board (we know Blue has a winning strategy by assumption), thus securing a Blue winning set. Notice that $p_2$ will be unable to obtain a red winning set, because it is not possible for the Blue and Red to obtain a winning configuration in a game of Hex. 


We will now show that other than claiming either $b_1$ or $b_2$, there is no other winning move for $p_1$. Suppose that $p_1$ claims either $b_3$ or an element from one of $Q_1, Q_2$, or $Q_3$. Then, $p_2$ will claim $r_1$, forcing $p_2$ to claim $b_1$. Then, $p_2$ will claim $b_2$. Now, $p_1$ will be unable to get any winning set, since $\{r_1, b_2\}$ intersects all winning sets.




So, suppose that $p_1$ as his first move claims either $r_1$ or $r_2$. Without loss of generality, assume that the first move was $r_1$. Then $p_2$ claims $b_1$. Now, if $p_1$ does not claim $r_2$, then $p_2$, by claiming $r_2$, will ensure that $p_1$ is unable to claim any winning set (since $\{b_1, r_2\}$ intersects all winning sets). So, $p_1$ must claim $r_2$. Now, $p_2$ claims $b_2$. Now, on the boards $Q_1, Q_2$, and $Q_3$, player $p_2$ will respond to each of $p_1$'s moves on a board according to Blue's winning strategy on that board (we know Blue has a winning strategy by assumption), thus securing a Blue winning set. Notice that $p_1$ will be unable to obtain a red winning set, because it is not possible for the Blue and Red to obtain a winning configuration in a game of Hex. Also, $p_1$ will be unable to obtain a blue winning set or a neutral winning set because $p_2$ has $b_1$ and $b_2$.

\end{proof}




\begin{lemma}
If red has a winning strategy in $Q$, then $p_1$ has at least one winning move, but claiming a $b_1$ or $b_2$ is not a winning move.
\end{lemma}
\begin{proof}


The winning strategy for $p_1$ is as follows. First, claim $r_1$. Now, $p_2$ is forced to claim $b_1$ (because $\{r_1, b_1\}$ is a winning set). Then, $p_1$ claims $r_2$, and $p_2$ is forced to claim $b_2$. Next, $p_1$ will by play a winning strategy for red on $Q_1$.
If $p_2$ plays on $Q_1$, then continue this strategy.
As soon as $p_2$ plays on a different board -- say, $Q_2$ -- then start playing a winning strategy for red on $Q_3$.
Thus $p_1$ will obtain red winning sets on two of the three boards.

So we have shown that $p_1$ has a winning strategy. We are left to show that $p_1$ does not have a winning strategy that starts with claiming either $b_1$ or $b_2$.


Suppose $p_1$ claims either $b_1$ or $b_2$ with their first move. Without loss of generality suppose that $p_1$ claimed $b_1$. Then $p_2$ responds by claiming $r_1$. Now, if $p_1$ does not claim $b_2$, then $p_2$ can force a draw (or win for $p_2$) by claiming $b_2$, since $\{r_1, b_2\}$ intersects all winning sets. So, $p_1$ claims $b_2$. Next, $p_2$ claims $r_2$. Now, if $p_1$ does not take $b_3$, then $p_2$ can force a draw (or win for $p_2$) by claiming $b_3$, since $\{r_1,r_2, b_3\}$ intersects all winning sets. So, $p_1$ claims $b_3$. Next, $p_2$ will by play a winning strategy for red on $Q_1$.
If $p_1$ plays on $Q_1$, then continue this strategy.
As soon as $p_1$ plays on a different board -- say, $Q_2$ -- then start playing a winning strategy for red on $Q_3$.
Thus $p_2$ will obtain red winning sets on two of the three boards.
\end{proof}

Together, these imply that we can determine the winning player in $Q$ by finding an optimal first move in the new symmetric maker-maker game (in particular, checking whether or not it is to take the blue element).
This completes the reduction.
\end{proof}

